VaLID: Variable-Length Input Diffusion for Novel View Synthesis

Novel View Synthesis (NVS), which tries to produce a realistic image at the target view given source view images and their corresponding poses, is a fundamental problem in 3D Vision. As this task is heavily under-constrained, some recent work, like Zero123, tries to solve this problem with generative modeling, specifically using pre-trained diffusion models. Although this strategy generalizes well to new scenes, compared to neural radiance field-based methods, it offers low levels of flexibility. For example, it can only accept a single-view image as input, despite realistic applications often offering multiple input images. This is because the source-view images and corresponding poses are processed separately and injected into the model at different stages. Thus it is not trivial to generalize the model into multi-view source images, once they are available. To solve this issue, we try to process each pose image pair separately and then fuse them as a unified visual representation which will be injected into the model to guide image synthesis at the target-views. However, inconsistency and computation costs increase as the number of input source-view images increases. To solve these issues, the Multi-view Cross Former module is proposed which maps variable-length input data to fix-size output data. A two-stage training strategy is introduced to further improve the efficiency during training time. Qualitative and quantitative evaluation over multiple datasets demonstrates the effectiveness of the proposed method against previous approaches. The code will be released according to the acceptance.

==> definitions.tex <==
\newcommand\ah[1]{\textcolor{green}{AmirH: #1}} %
\newcommand{\todo}[1]{{\textcolor{red}{#1}}}

==> figs/supp_qvis_2.tex <==


\begin{figure*}[t!]
\centering
\hspace{-5mm}
\subfloat[Target View]{
\begin{minipage}[t]{0.16\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/CITY_TAXI_POLICE_CAR_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/CITY_TAXI_POLICE_CAR_006.png}}\\
\vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/CITY_TAXI_POLICE_CAR_012.png}}\\
% \vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/CITY_TAXI_POLICE_CAR_015.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/PEEKABOO_ROLLER_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/PEEKABOO_ROLLER_007.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/PEEKABOO_ROLLER_022.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/GRANDFATHER_DOLL_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/Sootheze_Toasty_Orca_000.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/target/Sootheze_Toasty_Orca_009.png}}\\
\vspace{-3mm}
\end{minipage}
}
\hspace{-5mm}
\subfloat[Zero123\cite{liu2023zero}]{
\begin{minipage}[t]{0.16\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/CITY_TAXI_POLICE_CAR_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/CITY_TAXI_POLICE_CAR_006.png}}\\
\vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/CITY_TAXI_POLICE_CAR_012.png}}\\
% \vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/CITY_TAXI_POLICE_CAR_015.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/PEEKABOO_ROLLER_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/PEEKABOO_ROLLER_007.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/PEEKABOO_ROLLER_022.png}}\\
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/GRANDFATHER_DOLL_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/Sootheze_Toasty_Orca_000.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/zero123/Sootheze_Toasty_Orca_009.png}}\\
\vspace{-3mm}
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID (1 view)]{
\begin{minipage}[t]{0.16\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/CITY_TAXI_POLICE_CAR_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/CITY_TAXI_POLICE_CAR_006.png}}\\
\vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/CITY_TAXI_POLICE_CAR_012.png}}\\
% \vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/CITY_TAXI_POLICE_CAR_015.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/PEEKABOO_ROLLER_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/PEEKABOO_ROLLER_007.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/PEEKABOO_ROLLER_022.png}}\\
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/GRANDFATHER_DOLL_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/Sootheze_Toasty_Orca_000.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v1/Sootheze_Toasty_Orca_009.png}}\\
\vspace{-3mm}
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID (2 view)]{
\begin{minipage}[t]{0.16\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/CITY_TAXI_POLICE_CAR_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/CITY_TAXI_POLICE_CAR_006.png}}\\
\vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/CITY_TAXI_POLICE_CAR_012.png}}\\
% \vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/CITY_TAXI_POLICE_CAR_015.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/PEEKABOO_ROLLER_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/PEEKABOO_ROLLER_007.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/PEEKABOO_ROLLER_022.png}}\\
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/GRANDFATHER_DOLL_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/Sootheze_Toasty_Orca_000.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v2/Sootheze_Toasty_Orca_009.png}}\\
\vspace{-3mm}
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID (3 view)]{
\begin{minipage}[t]{0.16\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/CITY_TAXI_POLICE_CAR_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/CITY_TAXI_POLICE_CAR_006.png}}\\
\vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/CITY_TAXI_POLICE_CAR_012.png}}\\
% \vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/CITY_TAXI_POLICE_CAR_015.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/PEEKABOO_ROLLER_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/PEEKABOO_ROLLER_007.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/PEEKABOO_ROLLER_022.png}}\\
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/GRANDFATHER_DOLL_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/Sootheze_Toasty_Orca_000.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v3/Sootheze_Toasty_Orca_009.png}}\\
\vspace{-3mm}
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID (4 view)]{
\begin{minipage}[t]{0.16\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/CITY_TAXI_POLICE_CAR_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/CITY_TAXI_POLICE_CAR_006.png}}\\
\vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/CITY_TAXI_POLICE_CAR_012.png}}\\
% \vspace{-3mm}
% \includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/CITY_TAXI_POLICE_CAR_015.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/PEEKABOO_ROLLER_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/PEEKABOO_ROLLER_007.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/PEEKABOO_ROLLER_022.png}}\\
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/GRANDFATHER_DOLL_001.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/Sootheze_Toasty_Orca_000.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/supp/zero123_vs_valid/valid_v4/Sootheze_Toasty_Orca_009.png}}\\
\vspace{-3mm}
\end{minipage}
}
% \vspace{-3mm}
\caption{
More qualitative results.
}
\label{fig:qvis_2}
\vspace{-5mm}
\end{figure*} 


==> figs/supp_temporal_consistency_1.tex <==

\begin{figure*}[t!]
\centering
\subfloat[GT]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp3/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[Zero123]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp3/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID 1v]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp3/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID 4v]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp3/023.png}}\\
\end{minipage}
}
\subfloat[GT]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp4/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[Zero123]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp4/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID 1v]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp4/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID 4v]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp4/023.png}}\\
\end{minipage}
}
% \vspace{-3mm}
\caption{
Temporal consistency in the rendered video. The frames are in order from top to bottom.
}
\label{fig:temporal_consistency}
\vspace{-5mm}
\end{figure*} 



==> figs/supp_temporal_consistency_2.tex <==



\begin{figure*}[t!]
\centering
\subfloat[GT]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp1/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[Zero123]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp1/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID 1v]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp1/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID 4v]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp1/023.png}}\\
\end{minipage}
}
\subfloat[GT]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/gt/exp2/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[Zero123]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/zero123/exp2/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID 1v]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v1/exp2/023.png}}\\
\end{minipage}
}
\hspace{-5mm}
\subfloat[VaLID 4v]{
\begin{minipage}[t]{0.125\linewidth}
\centering
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/000.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/003.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/006.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/009.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/012.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/015.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/018.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/021.png}}\\
\includegraphics[width=\linewidth]
{{imgs/supp/video/VaLID_v4/exp2/023.png}}\\
\end{minipage}
}
% \vspace{-3mm}
\caption{
Temporal consistency in the rendered video.  The frames are in order from top to bottom.
}
\label{fig:motivation}
\vspace{-5mm}
\end{figure*} 



==> supplementary_arxiv.tex <==
\maketitlesupplementary

\input{figs/supp_zero123_cond}

\section{Conditioning Strategy}


As mentioned in the main paper, Zero123\cite{liu2023zero} is made of two conditioning mechanisms; (1) \emph{U-Net conditioning}, where a source-view image $x_i$ will go through a frozen Auto-Encoder and the output latent map $f^{AE}_i$ is then concatenated with a noisy latent feature map $z_t$ from the previous diffusion timestep $t+1$ as input to the U-Net. (2) \emph{Attention conditioning}, where the source-view image $x_i$ will go through a frozen CLIP image encoder. The output CLIP embedding $f^\mathrm{CLIP}_i$ is concatenated with the relative pose $\pi_i$ and then fed into the attention modules in the U-Net.

Figure~\ref{fig:cond} demonstrates the impacts of these two conditioning strategies on the generated images. 
To drop out the CLIP embedding, we mask them out with a 0-tensor of the same size.
It can be observed that in the case of following the default setting, where both U-Net conditioning and Attention conditioning exist, the model can produce plausible outcomes.
As a comparison, removing U-Net conditioning (w/o concat) produces poor outcomes, e.g. the objects in the generated images are usually in the wrong pose.
Moreover, the appearance of objects in generated images looks vastly different from the corresponding objects in the source-view images.
We hypothesize this is because the CLIP Image encoder can only output a single token for each input image which is a high-level semantic summary.
Thus, it is usually not enough to maintain image details.
By removing attention conditioning, we find the outcomes are almost the same, compared to the default setting.
This demonstrates U-Net conditioning dominates outcomes of Zero123 whereas CLIP embedding is almost ignored. 
% Surprisingly, in some examples, the generated images without attention conditioning preserve the textural information better.
% We hypothesize that this is because there are no conflicts between the two conditioning strategies.


% \section{Multi-view Consistency}

% To check the multi-view consistency among generated images, we conduct two experiments:
% \begin{itemize}
%     \item Temporal Consistency: We follow \cite{ye2023consistent} experiment setting. Specifically, we render a 24-frame video for each object and then check the temporal consistency inside the rendered video. This is evaluated by flow warping error $E_{wrap}$ \cite{lai2018learning}.
%     Specifically, we render a 24-frame video along a predefined camera trajectory and use RAFT \cite{teed2020raft} to compute the optical flow between two consecutive frames.
%     Then the error $E_{wrap}$ is defined as:
    
%     \begin{equation}
%         E_{wrap} = \sum_i ||x^i - \hat{x}^{i-1}||
%     \end{equation}

% where $\hat{x}^{i-1}$  is warped from the generated frame $x^{i-1}$ using the optical flow. 
%     \item Spatial Consistency: We follow \cite{watson2022novel} experiment setting. Specifically, for each object, we generate 100 images at random views. Then we train a NeRF with these images. Finally, we check the consistency between generated images from our model directly and rendered images from NeRF at validation views.
% \end{itemize}

% The results are shown in Table \ref{tab:res}. \textcolor{red}{Analysis}

% Finally, some qualitative results are shown in Figure \ref{fig:temporal_consistency}. We can observe the rendered video produced by the images generated from our method is with better consistency.

% \begin{table}[t]
%     \centering
%     \setlength{\tabcolsep}{3mm}
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{l|c|cccc}
%         \hline & Zero123$^*$ \cite{liu2023zero} & \multicolumn{4}{c}{MTDiff} \\
%         \hline
%         Input views & 1 & 1 & 2 & 3 & 4 \\
%         \hline 
%          Chamfer Dist. $\downarrow$ & 0.0054 & 0.0069 (0.0062) & 0.0045 & 0.0045 & 0.0041 (0.0046) \\
%         Volume IoU $\uparrow$ & 0.125 & 0.122 (0.104) & 0.118 & 0.132 & 0.127 (0.1181)\\
%         \hline
%         \end{tabular}
%         }
%     \caption{Training NeRF with generated images.}
%     \label{tab:res}
% \end{table}

% \begin{table}[t]
%     \centering
%     \setlength{\tabcolsep}{3mm}
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{l|c|llll}
%         \hline & Zero123$^*$ \cite{liu2023zero} & \multicolumn{4}{c}{VaLID} \\
%         \hline
%         Input views & 1      & 1     & 2     & 3     & 4v     \\
%         \hline
%         PSNR$\uparrow$  & 17.715 & 18.107 & 17.846 & 18.181 & 18.084 \\
%         L1$\downarrow$    & 1.004  & 0.977  & 0.982  & 0.902  & 0.905 
%         \end{tabular}
%     }
%     \caption{Optical flow consistency.}
%     \label{tab:optical_flow}
% \end{table}



\section{Qualitative Results}

Figure~\ref{fig:qvis_1} shows more qualitative results. It can be observed that compared to Zero123, our method can produce high-quality images.
In some examples, Zero123 produces objects in the wrong pose, the wrong shapes, or multiple objects whereas only a single object exists in the source-view images.
% As a comparison, the proposed \emph{VaLID} method can alleviate these issues.
This may be because there exists high uncertainty when only a single source-view image is available.
Unfortunately, Zero123 cannot handle this uncertainty well, especially when the difference between source-view and target-view is large.
Intuitively, the uncertainty usually decreases as the available information (source-view images) increases.
By receiving variable-length input views, the proposed method \emph{VaLID} can utilize multi-view image information thus producing high-quality images.
We can observe a clear improvement when the number of input views increases. 
Even if only a single source-view image is available, it can still outperform Zero123 qualitatively. 

To further demonstrate the utilization and fusion of multi-view input images by the proposed \emph{VaLID} method, Figure \ref{fig:stage} shows the generated images with or without stage 2 training.
As it can be observed in these examples, after stage 1 training, the model has the ability to produce plausible outcomes (see column (b)).
Although our model in stage 1 has the flexibility to receive variable-length input views, it has not been trained to fuse multi-view inputs. So, at this stage, the inference on multi-view inputs shows inconsistency in data fusion to generate reasonable output (see columns (c-e)).
In other words, since the training inputs in stage 1 of training always contain a single view image, the multi-view Cross Former block has not been adapted to perform the multi-view fusion task.
%This is because there exists inconsistency in the multi-view tokens which are fed into Multi-view Cross Former.
%Unfortunately, the Multi-view Cross Former does not come with the ability to deal with these inconsistencies.
%To solve this issue, we introduce stage 2 training.
To empower the model to perform the multi-view fusion, in stage 2 of training where only Cross Former parameters are tuned, the variable number of views are introduced as inputs.
With this efficient strategy, Multi-view Cross Former learns how to combine provided information from multiple images to generate a consistent output image.
%Furthermore, the Multi-view Cross Former can also fully utilize the information inside multiple source-view images.
As the number of input source-view images increases, the quality of produced images will gradually increase (see columns (f-i)).

Finally, we show some qualitative results in the attached video to show our method can produce more consistent images compared to previous methods.
These videos consist of generated images at a predefined camera trajectory.
We can observe with the single source-view image as input, that our method already can produce more consistent outcomes. When more input views are available, the consistency is improved further.


% \clearpage

% \subsection{Novel View Synthesis}

% \subsubsection{Multi-view Consistency}



% \textcolor{red}{More examples about Fig.~\ref{fig:motivation}}



% \subsection{3D Reconstruction}

% Furthermore, we also want to evaluate the multi-view consistency when multiple source-view images are available.
% This is evaluated by flow warping error $E_{wrap}$ \cite{lai2018learning}.
% Specifically, we render a 24-frame video along a predefined camera trajectory and use the RAFT \cite{teed2020raft} to compute the optical flow between two consecutive frames.
% Then the error $E_{wrap}$ is defined as:

% \begin{equation}
%     E_{wrap} = \sum_i ||x^i - \hat{x}^{i-1}||
% \end{equation}

% where $\hat{x}^{i-1}$  is warped from the generated frame $x^{i-1}$ using the optical flow. 

% We also apply our method to a 3D reconstruction pipeline.
% For this experiment, we measure Chamfer Distance and volumetric IoU on the reconstructed 3D point cloud.


% \begin{itemize}
%     \item Experiment Setting
%     \item Implementation details
    % \item Camera coordinate
    % \item Rendered video consistency
    % \item Training NeRF 
    % \item More qualitative results
    % \item Zero123 w/o CLIP, Concat
% \end{itemize}







% \input{figs/supp_temporal_consistency_1}
% \input{figs/supp_temporal_consistency_2}



















\input{figs/supp_qvis_1}
% \input{figs/supp_qvis_2}


\input{figs/supp_stage}

































==> texts/log/method_v0.tex <==
\section{Method}



We describe \method step-by-step.
We first start with a high-level overview of our method (Sec. \ref{sec:formulation}). Then we motivate our source view feature extractor (Sec. \ref{sec:feature_extraction}) and finally propose our extension to the multi-view setting (Sec. \ref{sec:multi_view_fusion}).
% Finally, a novel training strategy is proposed that allows for efficient training of our method (Sec. \ref{sec:training}).

\subsection{Overview}
\label{sec:formulation}
% \ya{I think we somewhere here need/want to mention that we wish to train with multiple inputs? }
%Previous work typically produces target-view images given only a single source-view image and in this work, we remove this restriction by proposing extend this to variable input views.
We aim for generating a realistic image $\boldsymbol{y}$ at the target-view, given any number of source-view images $\boldsymbol{x} = \{ x_i\}_{i=1}^{N_v}$, and corresponding camera poses relative to the target-view $\boldsymbol{\pi} = \{ \pi_i\}_{i=1}^{N_v}$, where $N_v\geq1$ is the chosen number of input source-view images.
To achieve this, two steps are involved: first extracting features from the source view images, then combining features from any number of source-view images $x_i$ to finally generate the target-view image either during training, inference or both.
A high-level figure is shown in \ref{fig:arch}.
In this work, we finetune a Visual image Transformer (ViT) architecture for extracting image features and combine them using our Multi-View CrossFormer module.
%The NVS is a heavily under-constrained task as there usually exists multiple plausible results for unobserved areas. We therefore utilize a diffusion model to handle this ambiguity to finally generate realistic target view images. 
The next sections go into detail on the different modules and training strategy.

\subsection{Source View Feature Extraction}
\label{sec:feature_extraction}
Following Zero123\cite{liu2023zero}, which can only accept a single source-view image $x_i$ and relative pose $\pi_i$ as input, we propose a ViT-based as an alternative feature extraction shown in Fig.~\ref{fig:overview}~(b). The introduced Source View Tokenization (SVT) module performs better feature extraction as well as enables us to extend it to the multi-view setting. 



Zero123 has two conditioning modules that we investigate. The first module is the \emph{U-Net conditioning}, where a source-view image $x_i$ will go through a frozen Auto-Encoder. The output latent map $f^{AE}_i$ is then concatenated with a noisy latent feature map $z_t$ from the previous diffusion timestep as input to the U-Net. Secondly, we have the \emph{Attention conditioning}, where the source-view image $x_i$ will go through a frozen CLIP image encoder. The output CLIP embedding $f^\mathrm{CLIP}_i$ is concatenated with the relative pose $\pi_i$ and then fed into the attention modules in the U-Net. Zero123\cite{liu2023zero} can thus be formulated as:
\begin{equation}
z_{t-1}=\boldsymbol{\epsilon}_\theta\left(f^{AE}_i \oplus z_t, {f^\mathrm{CLIP}_i} \oplus\pi_i, t\right), 
\label{eq:z123}
\end{equation}
where $\boldsymbol{\epsilon}_\theta$ denotes the U-Net,  $t$ the timestep in the diffusion process and symbol $\oplus$ denotes the concatenation operator.
% \ya{$CLIP$ is multiplying C with L with I etc. instead use $\text{CLIP}$ or  $\textsc{CLIP}$ or $f^\mathrm{CLIP}_i$ or something} are the latent feature map and CLIP embedding of source-view image $x$ separately.

We found the Attention conditioning to largely ignore the CLIP features and only propagates pose information as shown in Fig.~\ref{fig:motivation}. More examples are available in the supplemental materials.  We hypothesize that the CLIP encoding, a high-level single token image embedding, is too coarse to retain image details. Thus Eq.~(\ref{eq:z123}) reverts to $z_{t-1} \approx \boldsymbol{\epsilon}_\theta\left(f^{AE}_i \oplus z_t, \pi_i, t\right)$, where we see that the extracted features of input source-view image $f^{AE}_i$ and relative pose $\pi_i$ are injected into the U-Net at different stages.
This works well when only a single source-view image is available, like Zero123\cite{liu2023zero}.
However, when multiple source-view images are available, this disentangled appearance-pose strategy would require the model to align the poses with the source view features at a later stage in the network. 

Thus we propose to entangle appearance and pose features together. Since only U-Net conditioning encodes appearance information, one straightforward solution is that we feed both source-view images and corresponding poses to the U-Net input. The problem here is that the length of input views would be inherently tied to the first convolutional layer in the U-Net, making it inflexible. Furthermore, when multiple source-view images are available, feeding them directly into U-Net will produce inconsistent results which are shown in Fig.~\ref{fig:inconsistency}.
Thus we utilize the flexibility of attention mechanism and opt for feeding both source-view images and corresponding poses to the attention modules in U-Net.
In this way, we need to replace the CLIP image encoder by another architecture to better encode source-view images.
We achieve this with the $\mathbf{SVT}$ Module which can extract fine spatial information from source-view images.
% finetuning a Visual image Transformer architecture ($\mathbf{ViT}$).
Our final architecture can be formulated as:

% \begin{equation}
% z_{t-1}=\boldsymbol{\epsilon}_\theta\left(z_{t}, \bigoplus_{i=1}^{N_v} (\mathbf{SVT}(x_i) \oplus \pi_i), t\right)
% \end{equation}
\begin{equation}
z_{t-1}=\boldsymbol{\epsilon}_\theta\left(z_{t}, \mathbf{SVT}(x_1, \pi_1, ..., x_{N_{v}} , \pi_{N_{v}}), t\right)
\end{equation}

Then the network is trained by optimizing a simplified variational lower bound

\begin{equation}
    \mathcal{L} = \mathbb{E}[||\boldsymbol{\epsilon}_t - z_{t-1}||^2]
\end{equation}

% \begin{equation}
%     \mathcal{L} = \mathbb{E}[||\boldsymbol{\epsilon}_t - \boldsymbol{\epsilon}_\theta\left(z_{t}, \bigoplus_{i=1}^{N_v} (\mathbf{SVT}(x_i) \oplus \pi_i), t\right)||^2]
% \end{equation}
% \begin{equation}
% z_{t-1}=\boldsymbol{\epsilon}_\theta\left(\prod_{i=1}^{N_v} (\hat{x}^{s}_{i} || z_{t}), \prod_{i=1}^{N_v} \pi^s_i, t\right)
% \end{equation}
% where $\prod_{i=1}^{N_v}$ denotes $N_v$ source-view images are available.
%
% which can be formulated as:
% \begin{equation}
% z_{t-1}=\boldsymbol{\epsilon}_\theta\left(\prod_{i=1}^{N_v} (x_i || \pi^s_i) || z_{t}, t\right)
% \end{equation}

\begin{figure}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics{imgs/mvfusion.png}
    }
    \caption{Multi-view CrossFormer. During \textcolor{red}{\textbf{training}} time (stage 2), we randomly sample image tokens from all source-view images. With this strategy, we can make the Multi-view CrossFormer receives multi-view information while restrict training cost. In the \textcolor{green}{\textbf{inference}} time, we feed all the tokens to include all information.
    % \ya{ Already looks a lot better! Q: is the "xN" really inside the block or actually outside? it matters because depending on that we have multiple cross attentions or just multiple FFWs. if it's the latter, then put the "xN" closer to the FFW. Also: maybe make those black boxes different: one just includes data (inference/training) the other one is a new block. also: might be better to have "train" at the top and inference at the bottom! Also: just write out \texttt{concat} instead of this "c"}
    }
    \vspace{-5mm}
    \label{fig:mta}
\end{figure}

\begin{figure}[t]
\centering
\hspace{-5mm}
\subfloat[1 view]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp1_v0.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp2_v0.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp3_v0.png}}
\end{minipage}
}
\hspace{-5mm}
\subfloat[2 views]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp1_v01.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp2_v01.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp3_v01.png}}
\end{minipage}
}
\hspace{-5mm}
\subfloat[3 views]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp1_v012.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp2_v012.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp3_v012.png}}
\end{minipage}
}
\hspace{-5mm}
\subfloat[4 views]{
\begin{minipage}[t]{0.25\linewidth}
\centering
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp1_v0123.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp2_v0123.png}}\\
\vspace{-3mm}
\includegraphics[width=\linewidth]{{imgs/inconsistency/exp3_v0123.png}}
\end{minipage}
}
% \vspace{-3mm}
\caption{We can observe without the stage 2  training, there will exist heavily inconsistency in the outcomes when we feed multiple source-view images to the proposed architecture.}
\label{fig:inconsistency}
\vspace{-5mm}
\end{figure}   

\subsubsection{Source View Tokenization Module}
In the $\mathbf{SVT}$ Module, each input source-view pose image $(x_i, \pi_i)$ is processed separately and converted into pose-image tokens encoding both appearance and geometry information.
We extract features for each input source-view image $ x_i$ with a ViT.
Specifically, we adopt a pre-trained Masked Auto-Encoder (MAE)~\cite{he2022masked}.
The input image will be  converted into small image patches $\boldsymbol{\chi}= \{x_j\}_{j=1}^{N_{p}}$ where $N_{p}$ is the number of image patches. Positional embeddings are added to the images as in \cite{dosovitskiy2020image} for spatial awareness.
 Then these image patches are fed into MAE and converted into image tokens:

\begin{equation}
    \mathbf{M} =  \mathbf{MAE}(\boldsymbol{\chi}), \quad
    \mathbf{M} = \{m_j\}_{j=1}^{N_p}
\end{equation}
% \ya{ideally: don't use double letters to indicate variables etc. it's too easy to confuse with I*T.  maybe just use greek letters or something. sometimes using letters is ok, e.g. FF(X) or Attn(x) etc. but dont use it too often}
At this stage, each image token $m_j$ only contains appearance and 2D spatial information whereas camera pose information is missing.
To inject such information, the 3D poses are appended to the end of each token:
\begin{equation}
    \mathbf{\mathbf{\tilde{M}}} = \{ \tilde{m}_j \}_{j=1}^{N_p}, \text{where } \tilde{m}_j = m_j \oplus \pi^s .
\end{equation}
For now, each pose-image token $\tilde{m}_j$ is aware of both appearance information and spatial information (2D spatial and 3D pose).
Compared to the CLIP image encoder, the Source View Tokenization can extract rich spatial information and thus better describe image details. The proposed architecture is shown in Fig. \ref{fig:arch}.
Later, the extracted tokens from multiple source views can be fused together in our Multi-view Token Cross Former module described in the next Section.
\subsection{Multi View Fusion}
\subsubsection{Multi-view Cross Former}
\label{sec:multi_view_fusion}

In Source View Tokenization Module, we extract pose-image tokens $\mathbf{\tilde{M}}_i$ for each input source-view image.
As mentioned earlier, inconsistent results are produced when providing multi-views directly to the U-Net (Fig.~\ref{fig:inconsistency}).
% Thus a module for multi-view information fusion is needed. 
Alternatively feeding all large source view images tokens, will scale the computation proportionally to the number of images, and with attention having a complexity of $\mathcal{O}(N_v^2)$ this causes out of memory issues. Inspired by text-to-image diffusion models~\cite{rombach2022high}, where a fixed number of tokens have been shown to perform favorably, we introduce a fixed number (equal to 64) of learnable seed tokens $S_0$, initialized as $S_0 \sim N(0,1)$ at the beginning of training. These are used as queries in the multi-view cross former block, visualized in Fig. \ref{fig:mta}. Since these initial tokens $S_0$ are shared across training examples, they learn to be query token biases, which aim to extract relevant information from  pose-image tokens $\mathbf{\tilde{M}}_i$.
% However, this is only for one image as input. To fuse the information from multiple input source-view image, we propose multi-view token aggregation module which can merge multi-view information and produce an unified 3D representation shown in Fig. \ref{fig:mta}.
% One concern here is we hope our model can accept variable input views which may increase computation burden if the number of input views is large.
% To solve this issue, we initialize $N_{t}=64$ learnable seeds for target view $\mathbf{S} = \{s_l, i \in (1, N_{t})\}$ and gradually aggregate information from posed image tokens of input views as 3D representation $\mathbb{R}^{3D} = \{Tk_k, i \in (1, N_{p})\}$.
The multi-view cross former block, in particular, is first computed with an attention operation followed by a residual:
\begin{equation}
    \mathbf{S}'_{l} = \mathbf{Attn}_{l}(q, k, v) + \mathbf{S}_{l-1}.
\end{equation}
Then the output tokens will pass through a feed forward layer $\mathbf{FFW}_{l}$ which consists of layer normalization, a linear layer, GeLU activation, another linear layer sequentially, followed by a final residual connection:

\begin{equation}
    \mathbf{S}_l = \mathbf{FFW}_{l}(\mathbf{S}_l') + \mathbf{S}_l'.
\end{equation}

The query, key and value in the attention block are calculated with $q = \mathbf{S}_{l-1}$ and $\textbf{}k = v = \mathbf{\tilde{M}}_1 \oplus ... \oplus \mathbf{\tilde{M}}_{N_v}$.
The output tokens ${S}_l$ will be used as new target-view seeds for the following layer and the whole block will be repeated $L$ times. 
Finally the target-view seeds $S_L$  will be fed into attention modules at each timestep of the diffusion process to produce realistic images at the target view.
With this design, the final target-view seeds ${S}_L$ learns to warp the source view tokens into the target-view tokens that is being used for conditioning the diffusion process.
%With this design, we force the target-view seeds to learn the bias of the target-view information \hb{I don't know what this sentence means..}.
This also enables our model to always feed a fixed number of query tokens into the U-Net attention module, and brings the complexity of the attention down from $\mathcal{O}(N_v^2)$ to $\mathcal{O}(N_v)$.

% Then these patches are fed into visual transformer where they are converted into image tokens representing 3D structures.
% To utilize the recent progress of visual foundation model, we adopt Masked Auto-Encoder (MAE) and load its pretrained weights.
% The architecture of MAE is shown in Fig. \textcolor{red}{ref}.
% To make each image token being aware their pose information, we inject camera pose here by concatenating image tokens with their corresponding poses.
% At this stage each image token is being aware of their spatial location in 2D image and pose image in 3D space.

% One issue here is that each source-view image will produce 196 pose-image tokens.
% If multiple source-view images are available, there will be $196 \times N_v$ pose image tokens where $N_v$ is the number of input source-view images.
% Feeding such a large number pose-image tokens into attention modules will bring a heavy computation burden.
% To solve this issue, a token reduction strategy is required.
% This is achieved by an iterative module inspired by \cite{alayrac2022flamingo} which is shown in.
% To reduce the number of tokens to a fixed size, we initialize $N_{t}=64$ learnable tokens $LT = {LT_i, i \in (1, N_{t})}$.
% Then the information from pose-image tokens will be aggregated into these learnable tokens iteratively.
% This can be denoted as:



% \begin{equation}
%     \mathbf{FFW}() + x
% \end{equation}

% Finally, these image tokens will be fed into attention modules as key and value.

\subsubsection{Efficient Training and Inference strategy}
\label{sec:training}
As feeding multiple source-view images during training is still expensive, we split the whole training procedure into two steps.
In the first stage, the proposed architecture is trained to produce target-view images given a single source-view image.
After this stage, our model already has the ability to produce realistic target-view images.
As multi-view information aggregation only takes effect in Multi-view CrossFormer, we freeze all modules apart from  Multi-view CrossFormer in the second stage training.
With this strategy in the second stage of training, all the training resource will be used to make multi-view information work harmoniously to produce consistent outcomes. 
Additionally, we propose a sampling strategy during the second stage training where we feed a variable number of views to the model and randomly sample pose-image tokens from them.
By reducing the number of pose-image tokens fed into Multi-view CrossFormer, the training cost is further reduced.


\subsubsection{Stage 1: Single-view Optimization}
We build the proposed model on top of a pretrained stable-diffusion model. Thus we can assume the U-Net is already with the ability to produce realistic images. With this assumption, we only optimize the attention modules in the U-Net.
Thus in this stage, the Source View Tokenization Module, Multi-view CrossFormer and attention modules in the U-Net are optimized with a single source-view image as input.

\begin{figure*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics{imgs/example.pdf}
    }
    \vspace{-5mm}
    \caption{Qualitative results on GSO dataset. We can observe our method can produce high quality outcomes at the target-view compared to previous state-of-the-art method. Furthermore, the generated images from our method also maintain  consistency across different views. This is demonstrated by generated images along a predefined camera trajectory. Especially when multiple source-view images are available, the quality of generated images improves a lot.
    More examples can be found in the supplemental materials.}
    \label{fig:qvis_gso}
    % \vspace{-3mm}
\end{figure*}

\begin{table*}[h]
    \centering
    \setlength{\tabcolsep}{3mm}
    \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{l|cccc|cccc}
        \hline & DietNeRF~\cite{jain2021putting} & IV~\cite{sd-iv} & SJC-I~\cite{wang2023score}  & Zero123 \cite{liu2023zero} &  \multicolumn{4}{c}{\method} \\
        \hline
        View num & 1 & 1 & 1 & 1 & 1 & 2 & 3 & 4 \\
        \hline PSNR $\uparrow$ & $ 8.933$ & 5.914 & 6.573 & 19.000 &  20.034 & 20.405 & 21.053 & 21.305 \\
        SSIM $\uparrow$ & 0.645 & 0.540 & 0.552 &  0.865 & 0.881 & 0.884 & 0.891 & 0.895 \\
        LPIPS $\downarrow$ & $ 0.412 $ & 0.545 & 0.484 & 0.115 & 0.091 & 0.085 & 0.073 & 0.069 \\
        % FID $\downarrow$ & $\underline{12.919}$ & 22.533 & 19.783 & $\mathbf{0 . 0 2 7}$ \\
        % Dreamsim \cite{fu2023dreamsim} $\downarrow$ & - & - & - & - & \\
        \hline
        \end{tabular}
        }
    \caption{Results for novel view synthesis on Google Scanned Objects dataset. The proposed method outperforms previous state-of-the-art method by a  significant margin on all metrics. Furthermore, as the number of input source-view images increase, the performance gradually improved.}
    \label{tab:exp_gso}
    \vspace{-5mm}
\end{table*}

\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{3mm}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cccc|cccc}
        \hline & DietNeRF~\cite{jain2021putting} & IV~\cite{sd-iv} & SJC-I~\cite{wang2023score} & Zero123 \cite{liu2023zero}  & \method \\
        \hline
        Input views & 1 & 1 & 1 & 1 & 1\\
        \hline PSNR $\uparrow$ & 7.130 & 6.561 & 7.953  & 8.888 & 8.946\\
        SSIM $\uparrow$ & 0.406 & 0.442 & 0.456  & 0.513 & 0.515\\
        LPIPS $\downarrow$ & 0.507 & 0.564 & 0.545  & 0.438 & 0.433\\
        % FID $\dow         narrow$ & $\underline{\underline{5.143}}$ & 10.218 & 10.202 & $\mathbf{0 . 3 1 9}$ \\
        % Dreamsim \cite{fu2023dreamsim} $\downarrow$ & - & - & - & - & \\
        \hline
        \end{tabular}
        }
    \caption{Results for novel view synthesis on RTMV dataset. Compared to Google Scanned Objects dataset, this dataset contains more challenging scenes. We can observe our method still can outperfom other methods.}
    \label{tab:exp_rtmv}
    \vspace{-5mm}
\end{table}


\subsubsection{Stage 2: Variable-view Optimization}
After stage 1 training, we only finetune Multi-view CrossFormer where multi-view information fusion takes place. This is highlighted in ~\ref{fig:arch}
In each training iteration, variable input views are fed into the model while only partial pose-image tokens are fed into the U-Net for optimization
With this design, we not only improve the training efficiency due to feeding fewer pose-image tokens to the U-Net, but also improve the robustness of the proposed architecture when only partial information is available.
At inference time, we can choose to feed all pose-image tokens to the CrossFormer to provide more information to the model. We can alternatively sample less tokens for efficiency purposes bringing the complexity from $\mathcal{O}(N_v)$ to $\mathcal{O}(1)$, though we find thisalso hurts performance (shown in Sec.~\ref{sec:ablation}).


% we feed multiple source-view images as input to enable multi-view fusion ability of the proposed architecture.
% As at current stage, our architecture already with the ability of producing realistic images.
% Thus we only finetune the modules related to multi-view fusion.
% In our desing, we freeze the attention modules in U-Net as they are responsible for image generation and visual transformer architecture in Source View Tokenization Module as they are used to extract 3D representation from single-view image.
% With this strategy, we enforce the training focus on multi-view fusion while reduce trainable parameters a lot.
% To constrain the training burden, instead of feeding image tokens from all source-view images, we constrain image tokens with fixed number.
% This is achieved by uniformly sampling pose-image tokens from all source-view images.
% With this design, we also improve the roubustness of the proposed architectue when only partial information is available.


% 1. Fig 1: overview of Zero123 and ours

% 2. Fig2: architecture

% 3. Fig3. MAE

% 4. Fig4. Perceiver

% \subsection{Single-view Conditioning Synthesis}

% In this section, we will first illustrate how to apply the proposed architecture when only single-view image is available and then extend it to the setting that multiple source-view images are available.
% As the proposed architecture is based on previous work Zero123~\cite{liu2023zero}, we will first quickly present its architecture then highlights the main differences between them.

% \textbf{Zero123}
% The architecture of Zero123 is shown in Fig.~\ref{fig:overview} (a).
% Zero123 is a conditional diffusion model.
% By injecting a single-view image $\boldsymbol{x}^{\text {source }}$ and corresponding relative pose  $\boldsymbol{\pi}^{\text {source }}$, it can produce a realistic image at he target view iteratively 
% through a U-Net architecture starting from a noise map $\mathbf{\hat{x}^{s}}_T$.
% One thing needs to be noticed is Zero123 use a latent diffusion model where the U-Net operates on a latent map produced by a pretrained auto-encoder.
% The benefit of this design is that we can map high-dimension image data to a more compact feature space.
% For brevity, we still denote image in latent space with $x$ for the simplicity in the following.
% As mentioned previously, two steps are involved in this task, 3D content recovery from source-view image and target-view image generation.
% As Zero123 is a diffusion model, target-view image generation is achieved through U-Net iteratively.
% As for 3D content recovery, Zero123 utilize two different types of conditioning way in U-Net, U-Net conditioning and attention conditions, which are shown in From Fig.~\ref{fig:overview} (a). 
% In U-Net conditioning, the source-view image will first go through the auto-encoder.
% The output latent map is then concatenated with $z_t$ from previous timestep as input to the U-Net.
% As for attention conditioning, the source-view image will first go through a frozen CLIP image encoder.
% The pose information is injected here by concatenating the output CLIP embedding and relative pose.
% Finally, these features are fed into the attention modules in U-Net.
% Unfortunately, we found the attention conditioning degenerate to only inject pose information as Fig.~\ref{fig:motivation} shows.
% Thus in Zero123, U-Net is responsible to both 3D content recovery and target-view image generation.
% This entanglement limits the flexibility of Zero123, especially when multiple source-view images are available which is common in many realistic applications.
% This is because the pose information is injected in the attention modules while 3D representation is learnt in the U-Net which means it is difficult to build the correspondence between them.
% To solve this issue, we propose an architecture that can fully disentangle the conditioning and generation thus making utilizing multiple source-view images possible.

% \begin{equation}
% \hat{\boldsymbol{\epsilon}_t}=\boldsymbol{\epsilon}_\theta\left(\boldsymbol{y} \bigoplus \tilde{\boldsymbol{x}}^{\text {target }}, \boldsymbol{\pi}, t\right)
% \end{equation}

% The overview of the proposed architecture is shown in Fig.~\ref{fig:overview} (b).
% To disentangle 3D content recovery from target-view image generation, we remove the U-Net conditioning and only inject learnt 3D representation in the attention modules.
% To learn a 3D representation, we utilize a Visual Transformer architecture where we feed a single source-view image and get a image representation consisting of multiple image tokens.
% However, this representation is not aware their corresponding pose information.
% Here we simply concatenate them.
% To align this image representation to its corresponding 3D representation, we feed these tokens into the attention modules to produce realistic images at any target view.
% This will be illustrated later.

% \begin{equation}
%     x_{3D} = MAE(\tilde{\boldsymbol{x}}^{\text {target }} \bigoplus \boldsymbol{\pi}, t)
% \end{equation}

% \begin{equation}
% \hat{\boldsymbol{\epsilon}_t}=\boldsymbol{\epsilon}_\theta\left(\boldsymbol{y}, x_{3D} \right)
% \end{equation}

% he network is trained by optimizing a simplified variational lower bound
% \begin{equation}
%     \mathcal{L}_{\text {diffusion }}=\mathbb{E}\left[\left\|\boldsymbol{\epsilon}_t-\boldsymbol{\epsilon}_\theta\left(\boldsymbol{y}, \tilde{\boldsymbol{x}}^{\text {target }}, \hat{x}^{s}, t\right)\right\|^2\right]
% \end{equation}


% \subsection{Multi-view Fusion Module}

% In the above, we have already shown how to apply the proposed architecture when only single source-view image is available.
% In the following, I will hightlight how to apply the proposed architecture when multiple source-view images are available.
% Actually, this is achieved by a Multi-view Token Merging module (MTM) which is shown in Fig.~\ref{fig:mtm}.
% The output tokens from Source View Tokenization Module of single source-view image can be denoted as:
% \begin{equation}
%     \mathbf{M}k = \{ Tk_k \}, i \in \{1, N\}
% \end{equation}

% For the image tokens from multiple source-view images $\mathbf{M} = \{ \mathbf{M}k \}, k \in \{1, N\}$, we first concatenate them then feed them into the Multi-view Token Merging module.
% To aggregate information from multiple source-view images, MTM initialize $N$ learnable tokens where $N=64$ in this paper.
% Then we iteratively apply cross attention and feed forward operation on it where learnable tokens are used as query while $\mathbf{M}$ are used as key and value.

% \begin{equation}
%     \mathbf{Attn}(q, k, v)
% \end{equation}

% \begin{equation}
%     \mathbf{FFW}()
% \end{equation}

% \subsection{Efficient Two-stage training }

% For now, we already describe the whole architecture of the proposed architecture.
% However, there still exist one issue, efficient training.
% As there are many different modules in the proposed architecture where each of them takes different effect,
% What's worse, if we directly train the proposed model under multiple source-view setting, 


% \begin{equation}
% \hat{\boldsymbol{\epsilon}_t}=\boldsymbol{\epsilon}_\theta\left(\hat{x}^{s}^{source} \bigoplus \tilde{\boldsymbol{x}}^{\text {target }}, \boldsymbol{clip}^{source} \bigoplus \boldsymbol{\pi}, t\right)
% \end{equation}

% \begin{equation}
% \hat{\boldsymbol{\epsilon}_t}=\boldsymbol{\epsilon}_\theta\left(\Sigma_i^N (\hat{x}^{s}^{source}_i \bigoplus \tilde{\boldsymbol{x}}^{\text {target }}), \Sigma_i^N (\boldsymbol{clip}^{source}_i \bigoplus \boldsymbol{\pi}_i), t\right)
% \end{equation}

% \begin{equation}
% \hat{\boldsymbol{\epsilon}_t}=\boldsymbol{\epsilon}_\theta\left(\tilde{\boldsymbol{x}}^{\text {target }}, \boldsymbol{f}^{source} \bigoplus \boldsymbol{\pi}, t\right)
% \end{equation}

% \begin{equation}
% \hat{\boldsymbol{\epsilon}_t}=\boldsymbol{\epsilon}_\theta\left(\tilde{\boldsymbol{x}}^{\text {target }}, \Sigma_i^N (\boldsymbol{f}^{source}_i \bigoplus \boldsymbol{\pi}_i), t\right)
% \end{equation}




